Multimodal fusion of imaging and genomics for lung cancer recurrence prediction

Lung cancer has a high rate of recurrence in early-stage patients. Predicting the post-surgical recurrence in lung cancer patients has traditionally been approached using single modality information of genomics or radiology images. We investigate the potential of multimodal fusion for this task. By combining computed tomography (CT) images and genomics, we demonstrate improved prediction of recurrence using linear Cox proportional hazards models with elastic net regularization. We work on a recent non-small cell lung cancer (NSCLC) radiogenomics dataset of 130 patients and observe an increase in concordance-index values of up to 10%. Employing non-linear methods from the neural network literature, such as multi-layer perceptrons and visual-question answering fusion modules, did not improve performance consistently. This indicates the need for larger multimodal datasets and fusion techniques better adapted to this biological setting.

==> sections/conclusion.tex <==
\section{Conclusions}

From experiments on the limited dataset of 107 patients, we find that combining information from multiple modalities in the context of recurrence prediction in NSCLC shows promise.  Fusion techniques from VQA perform better than single modalities for NSCLC recurrence prediction despite originating in a different field. We believe that the development of fusion approaches with a deeper biological modelling between the different modalities could prove to be more effective. The availability of more paired datasets would be critical for a more rigorous comparison of the different fusion techniques' performance. 

While we worked with simpler feature extraction approaches from imaging and genomics, the use of more complex processing, including convolution networks with LSTMs to work with 3D radiology data and recurrent/graph neural networks to parse the genomics data, would be important to obtain the best fusion for NSCLC recurrence prediction. Given the limited size of the dataset, this would require the use of available single-modality datasets, such as those from TCGA for genomics followed by transfer learning. 

% 
% We believe that the poorer performance of the DenseNet features compared to the PyRadiomics features is due to the simplistic aggregation method across different slices. 

% We will explore the use of 3D convolutions directly on the nodule voxels instead of two-dimensional DenseNet on nodule slices. 
% This highlights the import



==> sections/experiments.tex <==
\section{Experiments and Results}

\begin{table*}[t]
\centering
\caption{C-Index comparisons of single modalities (genomics, DenseNet features, PyRadiomics features) vs multi-modality fusion. The fusion techniques of linear summation (Sum), concatenation (Concat), MFH~\cite{yu2018beyond}, and BLOCK~\cite{ben2019block} are evaluated for fusing genomics with DenseNet features, and PyRadiomics features. 5-fold cross validation is performed, and the best metrics are displayed for each fold. The average of the best scores is computed in the last column.
(Higher C-index is desired)}
\label{tab:results}\begin{tabular}{l|l|lllll|l}
Modalities                                                                          & Method             & Fold 1         & Fold 2         & Fold 3         & Fold 4         & Fold 5         & Average        \\ \hline
Genomics                                                                            & MLP(GenExp)        & 68.67          & 70.65          & 78.49          & 70.19          & 69.88          & 71.58          \\\hline
\multirow{2}{*}{Imaging}                                                            & MLP(PyRad)         & 75.90          & 77.17          & 63.44          & 72.12          & 80.72          & 73.87          \\
                                                                                    & MLP(DN)            & 73.49          & 78.26          & 73.12          & 75.96          & 77.11          & 75.59          \\\hline \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Genomics\\ +\\ PyRadiomics\end{tabular}} & Sum(Gen, PyRad)    & 81.93          & \textbf{82.61} & 75.27          & 73.08          & 75.90          & \textbf{77.76} \\
                                                                                    & Concat(Gen, PyRad) & 68.67          & 72.83          & 67.74          & 75.96          & 73.49          & 71.74          \\
                                                                                    & MFH(Gen, PyRad)    & 71.08          & 71.74          & 74.19          & 68.27          & 77.11          & 72.48          \\
                                                                                    & BLOCK(Gen, PyRad)  & 62.65          & 66.3           & 75.27          & 67.31          & \textbf{86.75} & 71.66          \\\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Genomics\\ +\\ DN features\end{tabular}} & Sum(Gen, DN)       & 74.70          & 75.00          & 74.19          & 75.96          & 68.67          & 73.71          \\
                                                                                    & Concat(Gen, DN)    & 69.88          & 69.57          & 70.97          & \textbf{76.92} & 78.31          & 73.13          \\
                                                                                    & MFH(Gen, DN)       & \textbf{87.95} & 72.83          & 70.97          & 75.96          & 72.29          & 76.00          \\
                                                                                    & BLOCK(Gen, PyRad)  & 74.70          & 73.91          & \textbf{79.57} & 74.04          & 71.08          & 74.66         \\ \hline
\end{tabular}
\end{table*}

We work with the NSCLC-Radiogenomics dataset~\cite{bakr2018radiogenomic}, which consists of 130 patients with information on gene expression, CT imaging, and recurrence information. Patients who underwent adjuvant/neo-adjuvant therapy in addition to surgical resection were removed from the patient cohort, yielding 107 patients.

The gene expression (RNAseq) data was available for all patients for 5268 genes. Each gene was preprocessed to lie in the range of 0 to 1. This served directly as the genomics feature vector.
The segmentations for nodules in the CT images were processed using the DICOM Toolkit dcmtk to obtain nodule masks for the nodules. These masks were fed into a standard radiomics library ~\cite{van2017computational} to obtain a 107-dimensional PyRadiomic (PyRad) features capturing texture and intensity patterns of the nodule and its immediate surrounding tissues of the lung. In addition, the different 2D slices within the mask area were processed through an Imagenet pretrained DenseNet~\cite{huang2017densely} to extract slice-level features, which were aggregated via max-pooling to obtain a 1024-dimensional DenseNet (DN) feature for each patient.  
A 5-fold cross validation was used with an 80-20 split for training and testing. 

\subsection{Results}

Our main focus was to compare single modality approaches to fusion approaches. The different methods we tested, shown in Fig.~\ref{fig:overview}, were all trained to minimize the survival loss function mentioned earlier with early stopping to avoid overfitting. We observed a range of variation in the C-Index values upon rerunning our model. Therefore, we performed 30 re-runs for each method and noted the best C-index values (shown in Table~\ref{tab:results}), alongside the distribution of values in Fig.~\ref{fig:box_plot}. 

To predict recurrence risk with single modalities, we used fully connected layers to construct multi-layer perceptrons, (MLP). 
To perform fusion, the imaging and genomic features were first processed separately through some fully connected layers, as shown in Fig.~\ref{fig:overview} to obtain a 256-dimensional feature vector for each modality. These were fused together by using the different methods to obtain a fused 256-dimensional feature vector, which was further fed through fully connected layers to predict risk of recurrence. 

The best C-index value using gene expression (GenExp) as inputs was 78.49, PyRadiomic features (PyRad) was 80.72 and DenseNet features (DN) was 78.26. The usage of fusion techniques greatly improved these numbers - the best genomics-PyRadiomics fusion methods earned the score of 86.75, while that of the best genomics-DenseNet fusion was 87.95.

When we look beyond the best values, to the distributions of the C-index values, we observe that the different methods share similar quartiles, as seen by the box edges in Fig.~\ref{fig:box_plot}. The range of the values is, however, considerably higher for two fusion methods - linear
summation with genomics-PyRadiomics and MFH with genomics-DenseNet features. This demonstrates the promise of fusion methods for recurrence prediction.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/box_plot.png}
    \caption{The range of different C-index values across different folds for the different methods of recurrence-risk prediction. Single modality in red, genomics and PyRadiomics features in light green, and genomics and DenseNet features in dark green.}
    \label{fig:box_plot}
\end{figure*}


==> sections/method.tex <==
\section{Methods}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/pipeline.png}
    \caption{Overview. We work with CT imaging and genomics of the same patient. We extract PyRadiomic and DenseNet features from the CT nodules, and work with gene expression data as is. We compare single modality MLP and four different multimodal fusion modules for NSCLC recurrence prediction. }
    \label{fig:overview}
\end{figure*}

\subsection{Fusion approaches}

Given data from multiple modalities, the fusion of information is a challenging problem of effectively identifying a better overall representation of the object of interest by appropriately weighting the different modalities. 
In our experiments, we employ two basic and two VQA-based fusion methods. 
The fusion block (shown in blue in Fig.~\ref{fig:overview}) takes as input, the imaging based feature $x \in \mathbb{R}^{256}$, and gene expression based feature $y \in \mathbb{R}^{256}$ to produce $z \in \mathbb{R}^{256}$ as follows:
% The fusion block (shown in blue in Fig.~\ref{fig:overview}) takes as input, the imaging based feature $x \in \mathbb{R}^{256}$, and gene expression based feature $y \in \mathbb{R}^{256}$ to produce $z \in \mathbb{R}^{256}$ as follows:
\begin{enumerate}[(i)]
    \setlength{\itemsep}{0em}
    \item (Sum) Linear Sum: $z = \text{ReLU}(F^{256: 256} (x + y) ) $
    \item (ConcatMLP) Concatenation + fully connected layer: $z = \text{ReLU}(F^{512: 256}([x, y])) $ 
    \item (MFH) Multimodal factorized higher-order pooling:  $z = \text{ReLU}( F_0^{l: 256}([z_0 \ , \ z_0 \ . \ z_1]) )$ where 
    $z_0 = F_1^{256: l} (x) \ . \ F_2^{256: l} (y)$ \ and \
    $z_1 = F_3^{256: l} (x)\ . \ F_4^{256: l} (y) $ 
    \item (BLOCK) Block superdiagonal tensor fusion: 
    $z = \text{ReLU}( \mathcal{T} \times x \times y )  ,$ where \\ $ \mathcal{T} = (\sum_{r=1}^R D_r \times X_r \times Y_r \times T_r)$
\end{enumerate}

where $F^{d_{\text{in}}:d_{\text{out}}}$ represents a fully connected layer with $d_{\text{in}}$ input channels and $d_{\text{out}}$ output channels. $[x, y]$ denotes concatenation, $F_0, F_1 \dots$ $F_4$ represent different fully connected layers. $D_r, X_r, Y_r, T_r$ are the different tensors for the filter decomposition, and $R$ is the rank of the decomposition. In our experiments, default values of $l$ and $R$ were used.

\subsection{Survival Analysis}
Survival analysis, similar to regression tasks, trains models to correctly assign a risk-value to each sample. However, unlike regression, it is not necessary that all patients in the dataset have experienced the event of interest. Each sample $i$ has two associated values:
\begin{enumerate}[(i)]
\setlength{\itemsep}{0em}
    \item A binary event value $e_i$, which indicates whether the patient experienced a recurrence ($e_i =$0) or no recurrence ($e_i =$ 1) in the study's observation period 
    \item An associated numeric value $t_i$ which equals the time duration of observation from surgery if there was no recurrence ($e_i = 0$), and the time to recurrence from surgery if there was a recurrence ($e_i = 1$). That is, $t_i = e_i (\text{time-to-recurrence}) + (1-e_i) (\text{time-under-observation})$
\end{enumerate}

% For example, a patient $i$ with no recurrence who was observed for 365 days has  $e_i = 0 $ and $t_i = 365$. Another patient $j$ who experienced recurrence on day 216 after surgery has $e_j = 1$ and $t_j = 216$.

Traditional methods to survival analysis, such as Cox proportional hazard models, have been evolving to include non-linearities in the form of neural networks. 
The survival loss function $\mathcal{L}(\mathbf{o})$, shown below, was proposed in~\cite{yao2017deep} to guide the network to predict risk scores $o_i$ for sample $i$, whose ordering agrees that of the ground truth events: 

$$\mathcal{L}(\mathbf{o}) = \sum_{i : e_i = 1} \Big(-o_i  + \log \sum_{j: t_j >= t_i} \exp (o_j) \Big) .$$

% An important property of this function is that it enables the use of all samples, including those for which the event is not observed.

\subsection{Concordance Index}


The concordance-index (C-index) is the most commonly used metric for survival analysis. It quantifies the effectiveness of a given risk-prediction algorithm in correctly ordering events. Consider values $\{e_i\}_{i=1}^N$, $\{t_i\}_{i=1}^N$ defined previously, $\{o_i\}_{i=1}^N$ the predicted recurrence risk-score for all $N$ patients in the data. It is desired to predict higher recurrence risk scores $o_i$ for patients with a lower $t_i$ if the recurrence was observed, $e_i = 1$. This is captured in the C-index, defined as
$$ \text{C-index} = \frac{1}{n} \sum_{i \in \{{1 \dots N : e_i = 1}\}} \sum_{t_j > t_i} \mathds{1}[o_i > o_j]. $$
A higher C-index value indicates that the method performs a better task at risk prediction.


% \subsection{Correlation (CCA)}

% \subsection{Interpretability - GradCAM and important genes}
